Totally Corrective Multiclass Boosting with Binary Weak Learners

In this work, we propose a new optimization framework for multiclass boosting learning. In the literature, AdaBoost.MO and AdaBoost.ECC are the two successful multiclass boosting algorithms, which can use binary weak learners. We explicitly derive these two algorithms' Lagrange dual problems based on their regularized loss functions. We show that the Lagrange dual formulations enable us to design totally-corrective multiclass algorithms by using the primal-dual optimization technique. Experiments on benchmark data sets suggest that our multiclass boosting can achieve a comparable generalization capability with state-of-the-art, but the convergence speed is much faster than stage-wise gradient descent boosting. In other words, the new totally corrective algorithms can maximize the margin more aggressively.

==> sect_expr.tex <==
%-------------------------------------------------------------------------
% \section{EXPERIMENTS} \label{Sec:Exps}

    In this section, we describe two sets of experiments
    to compare our new boosting algorithms with previous work.
    The first set makes use of decision stump as base learning method
    and the second uses linear discriminant analysis.
    The algorithms we compare include \MultiA{} and its stage-wise counterpart AdaBoost.MO,
    AdaBoost.ECC{} and its stage-wise counterpart AdaBoost.ECC.
    For \MultiA and AdaBoost.MO, we choose ECOC as the coding matrix.
    The dual optimization problems in new algorithms are solved
    by using the off-the-shelf MOSEK package \cite{mosek}.

%-------------------------------------------------------------------------
%\subsection{Experiments on UCI Datasets}

    %Table
    \setlength{\tabcolsep}{8pt}
    \begin{table}[!ht]
    \centering
    \caption{Multi-class UCI datasets}
    \label{table:datasets}
    \begin{tabular}{l|r|r|r|r}
    \hline%\toprule
    %\noalign{\smallskip}
        dataset & \#train & \#test & \#attribute & \#class \\
    %\noalign{\smallskip}
    \hline%\midrule
    %\noalign{\smallskip}
        svmguide2 & 391   & -    & 20 & 3  \\
        svmguide4 & 300   & 312  & 10 & 6  \\
        wine      & 178   & -    & 13 & 3  \\
        iris      & 150   & -    & 4  & 3  \\
        glass     & 214   & -    & 9  & 6  \\
        thyroid   & 3772  & 3428 & 21 & 3  \\
        dna       & 2000  & 1186 & 180 & 3 \\
        vehicle   & 846   & -    & 18 & 4  \\
    \hline%\bottomrule
    \end{tabular}
    \end{table}
    \setlength{\tabcolsep}{1.4pt}

    We collect $8$ datasets from UCI repository to run the experiments.
    A summary is listed in Table \ref{table:datasets}.
    If the dataset is provided with a pre-specified test set,
    we retain the partitioning setup,
    otherwise we use $70\%$ samples for training and the other $30\%$ for test.
    Validation sets are not required in our experiments. If needed,
    we do cross-validation directly on training sets.

    For each dataset, we merge the training set and test set,
    and rebuild them by random selection.
    Examples associated with the same class are carefully split in proportion
    to maintain the balance of multi-class problems.
    Then the boosting algorithms are trained and tested on new sets.
    For each dataset, this procedure is repeated $20$ times
    and the experimental results are averaged.

    The convergence threshold for \MultiA{} as well as \MultiB{} is set to $10^{-5}$.
    Another parameter to be tuned is the regularization parameter $\theta$,
    which equals to the $\Lone$ norm of weight vector associated with weak hypotheses.
    A simple method to choose $\theta$ is by running the corresponding stage-wise algorithms
    on the same data and compute the algebraic sum: $\theta = \sum_j \wj$.
    For datasets \svt, \svf, \win, \iri, \gla{} and \vow,
    which contain a small number of examples, we use this method;
    for the others, we do a five-fold cross validation to choose $\theta$
    from $\{ 2,5,8,10,12,15,20,30,40,45,60,80,100,120,150,200 \}$.

    The maximum number of training iterations is set to $50$, $100$ and $500$.
    For fairly comparison, we have forced our totally corrective boosting learning to run
    up to the maximum iteration even if the stopping criterion is satisfied.

    % Table
    \setlength{\tabcolsep}{8pt} %10pt for full page width
    \begin{table*}[!ht]
    \centering
    \caption{
        Training and test errors(including mean and standard deviation)
        of AdaBoost.MO, \MultiA, AdaBoost.ECC and \MultiB on UCI datasets.
        All results are averaged from $20$ tests.
        Base learners are decision stumps.
    }
    \label{table:dstump}
    %\newsavebox{\tablebox}
    %\begin{lrbox}{\tablebox}
    \begin{tabular}{llllllll}
    %
    %
    \hline
    dataset & algorithm
    		& train error 50	& train error 100	& train error 500
    		& test error 50	& test error 100	& test error 500	\\
    \hline
    	svmguide2
    	    &AB.MO	
    			& 0.016$\pm$0.005 	
    			& 0.000$\pm$0.000 	
    			& 0$\pm$0		
    			& 0.225$\pm$0.031 	
    			& \textbf{0.212$\pm$0.030 	}
    			& \textbf{0.221$\pm$0.021 	} \\
    	    &TC.MO	
    			& \textbf{0.011$\pm$0.003 	}
    			& \textbf{0$\pm$0		}
    			& 0$\pm$0		
    			& \textbf{0.224$\pm$0.024 	}
    			& 0.221$\pm$0.038 	
    			& 0.225$\pm$0.027 	 \\
    	\cline{2-8}
    	    &AB.ECC	
    			& 0.049$\pm$0.009 	
    			& 0.003$\pm$0.003 	
    			& 0$\pm$0		
    			& 0.253$\pm$0.032 	
    			& 0.226$\pm$0.031 	
    			& \textbf{0.216$\pm$0.031 	} \\
    	    &TC.ECC	
    			& \textbf{0.032$\pm$0.009 	}
    			& \textbf{0.001$\pm$0.002 	}
    			& 0$\pm$0		
    			& \textbf{0.242$\pm$0.031 	}
    			& \textbf{0.223$\pm$0.034 	}
    			& 0.221$\pm$0.028 	 \\
    \hline
    	svmguide4
    	    &AB.MO	
    			& 0.041$\pm$0.004 	
    			& 0.016$\pm$0.002 	
    			& 0$\pm$0		
    			& 0.204$\pm$0.025 	
    			& \textbf{0.194$\pm$0.017 	}
    			& \textbf{0.190$\pm$0.017 	} \\
    	    &TC.MO	
    			& \textbf{0.039$\pm$0.004 	}
    			& \textbf{0.014$\pm$0.002 	}
    			& 0$\pm$0		
    			& \textbf{0.203$\pm$0.023 	}
    			& 0.196$\pm$0.016 	
    			& 0.193$\pm$0.018 	 \\
    	\cline{2-8}
    	    &AB.ECC	
    			& 0.180$\pm$0.021 	
    			& 0.115$\pm$0.023 	
    			& 0$\pm$0		
    			& 0.285$\pm$0.023 	
    			& 0.262$\pm$0.025 	
    			& \textbf{0.233$\pm$0.023 	} \\
    	    &TC.ECC	
    			& \textbf{0.158$\pm$0.023 	}
    			& \textbf{0.087$\pm$0.020 	}
    			& 0$\pm$0		
    			& \textbf{0.275$\pm$0.022 	}
    			& \textbf{0.245$\pm$0.028 	}
    			& 0.237$\pm$0.022 	 \\
    \hline
    	wine
    	    &AB.MO	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.032$\pm$0.015 	
    			& \textbf{0.030$\pm$0.029 	}
    			& \textbf{0.031$\pm$0.028 	} \\
    	    &TC.MO	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.032$\pm$0.016 	
    			& 0.031$\pm$0.023 	
    			& 0.032$\pm$0.026 	 \\
    	\cline{2-8}
    	    &AB.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.026$\pm$0.020 	
    			& \textbf{0.034$\pm$0.028 	}
    			& \textbf{0.029$\pm$0.021 	} \\
    	    &TC.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.026$\pm$0.022 	
    			& 0.039$\pm$0.023 	
    			& 0.040$\pm$0.029 	 \\
    \hline
    	iris
    	    &AB.MO	
    			& 0.000$\pm$0.001 	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.062$\pm$0.026 	
    			& \textbf{0.064$\pm$0.025 	}
    			& 0.060$\pm$0.032 	 \\
    	    &TC.MO	
    			& \textbf{0$\pm$0		}
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& \textbf{0.062$\pm$0.026 	}
    			& 0.067$\pm$0.023 	
    			& \textbf{0.057$\pm$0.025 	} \\
    	\cline{2-8}
    	    &AB.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& \textbf{0.057$\pm$0.024 	}
    			& \textbf{0.061$\pm$0.018 	}
    			& \textbf{0.049$\pm$0.027 	} \\
    	    &TC.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.061$\pm$0.021 	
    			& 0.067$\pm$0.020 	
    			& 0.060$\pm$0.027 	 \\
    \hline
    	glass
    	    &AB.MO	
    			& 0.026$\pm$0.003 	
    			& 0.003$\pm$0.001 	
    			& 0$\pm$0		
    			& \textbf{0.275$\pm$0.034 	}
    			& \textbf{0.246$\pm$0.061 	}
    			& \textbf{0.268$\pm$0.051 	} \\
    	    &TC.MO	
    			& \textbf{0.022$\pm$0.003 	}
    			& \textbf{0.002$\pm$0.001 	}
    			& 0$\pm$0		
    			& 0.280$\pm$0.039 	
    			& 0.252$\pm$0.059 	
    			& 0.273$\pm$0.047 	 \\
    	\cline{2-8}
    	    &AB.ECC	
    			& 0.168$\pm$0.032 	
    			& 0.078$\pm$0.018 	
    			& 0$\pm$0		
    			& 0.352$\pm$0.052 	
    			& 0.313$\pm$0.043 	
    			& \textbf{0.284$\pm$0.051 	} \\
    	    &TC.ECC	
    			& \textbf{0.113$\pm$0.030 	}
    			& \textbf{0.020$\pm$0.013 	}
    			& 0$\pm$0		
    			& \textbf{0.327$\pm$0.048 	}
    			& \textbf{0.302$\pm$0.035 	}
    			& 0.298$\pm$0.052 	 \\
    \hline
    	thyroid
    	    &AB.MO	
    			& \textbf{0.003$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		
    			& \textbf{0.004$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	    &TC.MO	
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	\cline{2-8}
    	    &AB.ECC	
    			& \textbf{0.008$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		
    			& \textbf{0.007$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	    &TC.ECC	
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		 \\
    \hline
    	dna
    	    &AB.MO	
    			& \textbf{0.051$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		
    			& \textbf{0.082$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	    &TC.MO	
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	\cline{2-8}
    	    &AB.ECC	
    			& \textbf{0.062$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		
    			& \textbf{0.094$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	    &TC.ECC	
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		 \\
    \hline
    	vehicle
    	    &AB.MO	
    			& 0.098$\pm$0.004 	
    			& 0.071$\pm$0.003 	
    			& 0.017$\pm$0.003 	
    			& 0.258$\pm$0.026 	
    			& 0.243$\pm$0.026 	
    			& 0.230$\pm$0.019 	 \\
    	    &TC.MO	
    			& \textbf{0.093$\pm$0.003 	}
    			& \textbf{0.066$\pm$0.003 	}
    			& \textbf{0.013$\pm$0.002 	}
    			& \textbf{0.253$\pm$0.024 	}
    			& \textbf{0.240$\pm$0.023 	}
    			& \textbf{0.227$\pm$0.019 	} \\
    	\cline{2-8}
    	    &AB.ECC	
    			& 0.271$\pm$0.010 	
    			& 0.205$\pm$0.004 	
    			& N$\pm$N		
    			& 0.359$\pm$0.022 	
    			& 0.296$\pm$0.006 	
    			& N$\pm$N		 \\
    	    &TC.ECC	
    			& \textbf{0.208$\pm$0.018 	}
    			& \textbf{0.145$\pm$0.013 	}
    			& N$\pm$N		
    			& \textbf{0.327$\pm$0.022 	}
    			& \textbf{0.271$\pm$0.002 	}
    			& N$\pm$N		 \\
    \hline
    %
    %
    \end{tabular}
    %\end{lrbox}
    % \resizebox{120mm}{!}{\usebox{\tablebox}}
    \end{table*}
    \setlength{\tabcolsep}{1.4pt}

    %figure1
    \begin{figure*}[h!]
    \begin{center}
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train1}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train2}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train3}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train4}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train5}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train6}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train7}
        }
        \subfigure[]
        {
            \includegraphics[width=0.20\textwidth,clip]{glass_TRN}
            \label{fig:train8}
        }
    \end{center}
    \caption
    {
        Training error curves of AdaBoost.MO, \MultiA, AdaBoost.ECC and \MultiB
        on \gla, \gla, \gla, \gla, \gla and \gla.
        The results are averaged from $20$ tests.
        Decision stumps are used as base learners.
	}
    \label{fig:train}
    \end{figure*}

    First we use decision stump as the base learning method for all algorithms.
    The experimental results are reported in Table \ref{table:dstump}.
    As we can see, all the training errors of new algorithms are better
    than their counterparts, except for the case both algorithms have converged to $0$.
    We show the training error curves of $6$ datasets in Fig. \ref{fig:train},
    where the maximum number of training iterations is $500$.
    The convergence speed of our totally corrective boosting algorithm
    is clearly faster than the stage-wise one.
    This conclusion is consistent with the discussion in Section \ref{sec:ecc-dual}.
    A fast convergence speed is beneficial to reduce the training cost
    and in some cases, it also helps to produce a simpler classifier
    which consists of fewer weak hypotheses \cite{viola2004robust}.


    In terms of test error, new algorithms are better than their counterparts
    on $6$ datasets but worse on the other $2$. Empirically speaking,
    new algorithm has a comparable generalization ability with the original one.
    However, it is noticeable that on \thy, \dna{} and \veh


    In the second set of experiments,
    we use Fisher's linear discriminant function as the base learner.
    MO and ECC comparison. why do not run MO in the second experiment
    (K times more variables if solving dual optimization).


    %figure2
    \begin{figure*}[]
    \begin{center}
        \subfigure[]
        {
            \includegraphics[width=0.30\textwidth,clip]{glass_TST}
            \label{fig:test1}
        }
        \subfigure[]
        {
            \includegraphics[width=0.30\textwidth,clip]{glass_TST}
            \label{fig:test2}
        }
        \subfigure[]
        {
            \includegraphics[width=0.30\textwidth,clip]{glass_TST}
            \label{fig:test3}
        }
        \subfigure[]
        {
            \includegraphics[width=0.30\textwidth,clip]{glass_TST}
            \label{fig:test4}
        }
        \subfigure[]
        {
            \includegraphics[width=0.30\textwidth,clip]{glass_TST}
            \label{fig:test5}
        }
        \subfigure[]
        {
            \includegraphics[width=0.30\textwidth,clip]{glass_TST}
            \label{fig:test6}
        }
    \end{center}
    \caption
    {
        Test error curves of AdaBoost.MO, \MultiA, AdaBoost.ECC and \MultiB.
        The results are averaged from $20$ tests.
        Decision stumps are used as base learners.
	}
    \label{fig:test}
    \end{figure*}

    % Table2
    \setlength{\tabcolsep}{8pt} %10pt for full page width
    \begin{table*}[!t]
    \centering
    \caption{
        Training and test errors (including mean and standard deviation)
        of AdaBoost.ECC and \MultiB.
        All results are averaged from 20 times tests.
        Base learners are Fisher's linear discriminant functions.
    }
    \label{table:lda}
    %\newsavebox{\tablebox}
    %\begin{lrbox}{\tablebox}
    \begin{tabular}{llllllll}
    %
    %
    \hline
    dataset & algorithm
    		& train error 50	& train error 100	& train error 500
    		& test error 50	& test error 100	& test error 500	\\
    \hline
    	svmguide2
    	    &AB.ECC	
    			& 0.049$\pm$0.009 	
    			& 0.003$\pm$0.003 	
    			& 0$\pm$0		
    			& 0.253$\pm$0.032 	
    			& 0.226$\pm$0.031 	
    			& \textbf{0.216$\pm$0.031 	} \\
    	    &TC.ECC	
    			& \textbf{0.032$\pm$0.009 	}
    			& \textbf{0.001$\pm$0.002 	}
    			& 0$\pm$0		
    			& \textbf{0.242$\pm$0.031 	}
    			& \textbf{0.223$\pm$0.034 	}
    			& 0.221$\pm$0.028 	 \\
    \hline
    	svmguide4
    	    &AB.ECC	
    			& 0.180$\pm$0.021 	
    			& 0.115$\pm$0.023 	
    			& 0$\pm$0		
    			& 0.285$\pm$0.023 	
    			& 0.262$\pm$0.025 	
    			& \textbf{0.233$\pm$0.023 	} \\
    	    &TC.ECC	
    			& \textbf{0.158$\pm$0.023 	}
    			& \textbf{0.087$\pm$0.020 	}
    			& 0$\pm$0		
    			& \textbf{0.275$\pm$0.022 	}
    			& \textbf{0.245$\pm$0.028 	}
    			& 0.237$\pm$0.022 	 \\
    \hline
    	wine
    	    &AB.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.026$\pm$0.020 	
    			& \textbf{0.034$\pm$0.028 	}
    			& \textbf{0.029$\pm$0.021 	} \\
    	    &TC.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.026$\pm$0.022 	
    			& 0.039$\pm$0.023 	
    			& 0.040$\pm$0.029 	 \\
    \hline
    	iris
    	    &AB.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& \textbf{0.057$\pm$0.024 	}
    			& \textbf{0.061$\pm$0.018 	}
    			& \textbf{0.049$\pm$0.027 	} \\
    	    &TC.ECC	
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0$\pm$0		
    			& 0.061$\pm$0.021 	
    			& 0.067$\pm$0.020 	
    			& 0.060$\pm$0.027 	 \\
    \hline
    	glass
    	    &AB.ECC	
    			& 0.168$\pm$0.032 	
    			& 0.078$\pm$0.018 	
    			& 0$\pm$0		
    			& 0.352$\pm$0.052 	
    			& 0.313$\pm$0.043 	
    			& \textbf{0.284$\pm$0.051 	} \\
    	    &TC.ECC	
    			& \textbf{0.113$\pm$0.030 	}
    			& \textbf{0.020$\pm$0.013 	}
    			& 0$\pm$0		
    			& \textbf{0.327$\pm$0.048 	}
    			& \textbf{0.302$\pm$0.035 	}
    			& 0.298$\pm$0.052 	 \\
    \hline
    	thyroid
    	    &AB.ECC	
    			& \textbf{0.008$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		
    			& \textbf{0.007$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	    &TC.ECC	
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		 \\
    \hline
    	dna
    	    &AB.ECC	
    			& \textbf{0.062$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		
    			& \textbf{0.094$\pm$0.000 	}
    			& N$\pm$N		
    			& N$\pm$N		 \\
    	    &TC.ECC	
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		
    			& N$\pm$N		 \\
    \hline
    	vehicle
    	    &AB.ECC	
    			& 0.271$\pm$0.010 	
    			& 0.205$\pm$0.004 	
    			& N$\pm$N		
    			& 0.359$\pm$0.022 	
    			& 0.296$\pm$0.006 	
    			& N$\pm$N		 \\
    	    &TC.ECC	
    			& \textbf{0.208$\pm$0.018 	}
    			& \textbf{0.145$\pm$0.013 	}
    			& N$\pm$N		
    			& \textbf{0.327$\pm$0.022 	}
    			& \textbf{0.271$\pm$0.002 	}
    			& N$\pm$N		 \\
    \hline
    %
    %
    \end{tabular}
    %\end{lrbox}
    % \resizebox{120mm}{!}{\usebox{\tablebox}}
    \end{table*}
    \setlength{\tabcolsep}{1.4pt}%1.4 originally

%-------------------------------------------------------------------------
\subsection{Experiments on Face recognition}

    Eigenface 
